DADA: Dual Averaging with Distance Adaptation

We present a novel universal gradient method for solving convex optimization problems. Our algorithm, Dual Averaging with Distance Adaptation (DADA), is based on the classical scheme of dual averaging and dynamically adjusts its coefficients based on observed gradients and the distance between iterates and the starting point, eliminating the need for problem-specific parameters. DADA is a universal algorithm that simultaneously works for a broad spectrum of problem classes, provided the local growth of the objective function around its minimizer can be bounded. Particular examples of such problem classes are nonsmooth Lipschitz functions, Lipschitz-smooth functions, H\"older-smooth functions, functions with high-order Lipschitz derivative, quasi-self-concordant functions, and $(L_0,L_1)$-smooth functions. Crucially, DADA is applicable to both unconstrained and constrained problems, even when the domain is unbounded, without requiring prior knowledge of the number of iterations or desired accuracy.

==> Applications/holder_smooth_functions.tex <==
\paragraph{H\"older-smooth functions.}
The previous two examples are subclasses of the more general class of
H\"older-smooth functions. It is defined by the following inequality:
\begin{align*}
  \dnorm{\nabla f(x) - \nabla f(y)} \le H_{\nu} \norm{x - y}^{\nu}
\end{align*}
for all $x, y \in \R^d$, where $\nu \in [0, 1]$ and $H_{\nu} \geq 0$.
Therefore, for $\nu = 0$, we get functions with bounded variation of
subgradients (which contains all Lipschitz functions) and for $\nu = 1$ we get
Lipschitz-smooth functions.

The complexity of DADA on this problem class is
(see \cref{thm:holder-smooth-convergence})
\begin{align*}
  \BigO\biggl(
    \biggl[\frac{H_{\nu}}{\epsilon}\biggr]^{\frac{2}{1 + \nu}} \bar{D}_0^2
    \log_{+}^{2}\frac{\bar{D}_0}{\Bar{r}}
  \biggr).
\end{align*}
This is similar to the
$\BigO\bigl(\bigl[\frac{H_{\nu}}{\epsilon}\bigr]^{\frac{2}{1 + \nu}} D_0^2 +
    \log \Abs[\big]{
      \frac{H_{\nu}^{\frac{2}{1 + \nu}}}{\hat{L} \epsilon^{\frac{1 - \nu}{1 + \nu}}}
    }
  \bigr)$
complexity of the universal (nonaccelerated)
gradient method with line search (GM-LS)~\cite{Nesterov2015UniversalGM},
where $\hat{L}$ is the parameter of the method.
Again, the complexity of GM-LS is slightly
better since the logarithmic factor is additive (and not multiplicative).
However, GM-LS is not guaranteed to work (well)
on other problem classes such as those we consider next.


==> Applications/l0_l1_smooth_functions.tex <==
\paragraph{$(L_0, L_1)$-smooth functions.}
As introduced in \cite{Zhang2020Why},
a function $f$ is said to be $(L_0, L_1)$-smooth
if for all $x \in \R^d$, we have
\[
  \norm{\nabla^2 f(x)} \le L_0 + L_1 \dnorm{\nabla f(x)}.
\]
The complexity of DADA on this class is
(see \cref{thm:l0-l1-smooth-convergence})
\begin{align*}
  \BigO\biggl(
    \left[
      L_1^2 \bar{D}_0^2
      +
      \frac{L_0 \bar{D}_0^2}{\epsilon}
    \right]
    \log_+^2 \frac{\bar{D}_0}{\Bar{r}}
  \biggr).
\end{align*}
Up to the extra logarithmic factor, this matches the complexity of NGM from
\cite{Vankov2024OptimizingL0L1SmoothFunctions},
with the distinction that their approach is less robust to the initial guess
of $D_0$. Specifically, the penalty for underestimating it in the latter
method is a multiplicative factor of
$\rho^2 \DefinedEqual \frac{D_0^2}{\bar{r}^2}$ while in our method this factor
is logarithmic: $\log_+^2 \rho$.


==> Applications/lipschitz_highorder_derivative_functions.tex <==
\paragraph{Functions with Lipschitz high-order derivative.}

This class is a generalization of the Lipschitz-smooth class.
Functions in this class are $p$ times differentiable, and
have the property that their $p$th derivative ($p \geq 2$)
is Lipschitz, i.e., for all $x, y \in \R^d$,
we have
\begin{align*}
  \norm{\nabla^{p} f(x) - \nabla^{p} f(y)} \le L_{p} \norm{x - y},
\end{align*}
where the $\norm{\cdot}$ norm in the left-hand side is
the usual operator norm of a symmetric $p$-linear operator:
$\norm{A} = \max_{h \in \R^d \colon \norm{h} = 1} \norm{A[h]^p}$.
For example, the $p$th power of the Euclidean norm is an example of a function
in this class (see~\cite{Rodomanov2019SmoothnessPO}). The complexity of DADA on
this problem class is
(see \cref{thm:high-order-derivative-lipschitz-convergence})
\begin{align*}
  \BigO\biggl(
    \biggl[
      \max_{2 \le i \le p} \biggl[\frac{p}{i!} \frac{\dnorm{\nabla^i
            f(x^*)}}{\epsilon}\biggr]^{\frac{2}{i}} +
      \biggl[\frac{L_p}{p! \, \epsilon}\biggr]^{\frac{2}{p + 1}}
    \biggr]
    \bar{D}_0^2 \log_{+}^{2}\frac{\bar{D}_0}{\Bar{r}}
  \biggr).
\end{align*}
Although line-search gradient methods might be better for
H\"older-smooth problems, to our knowledge,
they are not known to attain comparable bounds on this function class.


==> Applications/lipschitz_smooth_functions.tex <==
\paragraph{Lipschitz-smooth functions.}

Another important class of functions are those with Lipschitz gradient:
\begin{align*}
  \dnorm{\nabla f(x) - \nabla f(y)} \leq L_1 \norm{x - y}
\end{align*}
for all $x, y \in \R^d$.
In this case, the complexity of our method is
(see \cref{thm:lipschitz-smooth-convergence})
\begin{align*}
  \BigO\left(
    \frac{L_1 \bar{D}_0^2}{\epsilon} \log_{+}^2 \frac{\bar{D}_0}{\bar{r}}
  \right).
\end{align*}
This coincides with the standard complexity of the (nonaccelerated) gradient
method on Lipschitz-smooth
functions~\cite[Section~3]{Nesterov2018LecturesOnCVX}
up to an extra logarithmic factor.

Note that the complexity of DADA is slightly worse than that of the classical
gradient method with line search
\cite{Nesterov2015UniversalGM}, which achieves a complexity bound of
$\BigO\bigl(\frac{L_1 D_0^{2}}{\epsilon} + \log
    \Abs[\big]{\frac{L_1}{\hat{L}_1}}\bigr)$,
where $\hat{L}_1$ is the initial guess for $L_1$.
The difference is that the logarithmic factor in the latter estimate appears
in an additive way instead of multiplicative.


==> Applications/nonsmooth_lipschitz_functions.tex <==
\paragraph{Nonsmooth Lipschitz functions.}

This function class is defined by the inequality
\begin{align*}
  \abs{f(x) - f(y)} \leq L_0 \norm{x - y}
\end{align*}
for all $x, y \in \R^d$.
For this problem class, DADA requires at most
(see \cref{thm:nonsmooth-lipschitz-convergence})
\begin{align*}
  \BigO\left(
    \frac{L_0^2 \bar{D}_0^2}{\epsilon^2}\log_{+}^2 \frac{\bar{D}_0}{\Bar{r}}
  \right)
\end{align*}
oracle calls to reach $\epsilon$-accuracy,
which matches the standard complexity of (sub)gradient
methods~\cite{Nesterov2005PrimaldualSM, Nesterov2018LecturesOnCVX},
up to an extra logarithmic factor.
Note that a polylogarithmic factor in
$\frac{\bar{D}_0}{\bar{r}}$
appears in the complexity bounds of all distance-adaptation
methods~\cite{Defazio2023DAdaptation,Ivgi2023DoGIS,Khaled2023DoWG,Mishchenko2024Prodigy}.


==> Applications/quasi_self_concordant_functions.tex <==
\paragraph{Quasi-self-concordant (QSC) functions \cite{Bach2010SelfConcordant}.}
A function~$f$ is called QSC with parameter $M \geq 0$
if it is three times continuously differentiable and the following inequality
holds for any $x, u, v \in \R^d$:
\begin{align}\label{eq:qsc}
  \nabla^3 f(x)[u, u, v] \le M \inp{\nabla^2 f(x)u}{u} \norm{v}.
\end{align}
For example, the exponential, logistic, and softmax functions are QSC; for
more details and other examples, see \cite{Doikov2023QuasiSelfConcordant}.
When applied to a QSC function, our method has the following complexity
(\cref{thm:qsc-convergence}):
\begin{align*}
  \BigO\biggl(
    \left[
      M^2 \bar{D}_0^2
      +
      \frac{\norm{\nabla^2 f(x^*)} \bar{D}_0^2}{\epsilon}
    \right]
    \log_{+}^2 \frac{\bar{D}_0}{\Bar{r}}
  \biggr).
\end{align*}
In terms of comparisons, second-order methods, such as those explored in
\cite{Doikov2023QuasiSelfConcordant}, are more powerful for minimizing QSC
functions, as they leverage additional curvature information. Their complexity
bound, in terms of queries to the second-order oracle, is
$\BigO(
    M \hat{D}_0
    \log \frac{F_0}{\epsilon} + \log \frac{\hat{D}_0 g_0}{\epsilon F_0}
  )$, where $F_0 = f(x_0) - f^*$, $\hat{D}_0$ is the
diameter of the initial sublevel set, and $g_0 = \dnorm{\nabla f(x_0)}$
(see~\cite[Corollary 3.4]{Doikov2023QuasiSelfConcordant}). However, each
iteration of these methods is significantly more expensive.

To our knowledge, the QSC class has not been previously studied in the
context of first-order methods. The only other first-order methods for which
one can prove similar bounds are the nonadaptive variants of our scheme,
namely the normalized gradient method (NGM) from
\cite[Section~5]{Nesterov2018LecturesOnCVX} and
the recent improvement of this algorithm for constrained
problems~\cite{Nesterov2024PredfinedStep}.


==> Experiments/worst_case_function.tex <==
\paragraph{Worst-case function.}
As an example of a function with Lipschitz high-order derivative, we consider
the following worst-case problem from \cite{Doikov2024SuperUniversal}:
\begin{align}
  \min_{x \in \R^d} \Bigl\{
    f(x)
    \DefinedEqual
    \frac{1}{p} \sum_{i = 1}^{d - 1}
    \Abs{x\UpperIndex{i} - x\UpperIndex{i + 1}}^p
    +
    \frac{1}{p} \Abs{x\UpperIndex{d}}^p
  \Bigr\},
\end{align}
where $p \geq 2$, and $x\UpperIndex{i}$ is the $i$th element of~$x$.
The optimal point in this problem is $x^* = 0$.

\begin{figure}[tb]
  \centering
  \includegraphics[width=\textwidth]{Figures/comparison-WI-residual.pdf}
  \caption{
    Comparison of different methods on the worst-case function.
  }
  \label{fig:worst-instance-residual}
\end{figure}

As illustrated in \cref{fig:worst-instance-residual},
nearly all methods exhibit similar performance when $p = 2$,
except for Prodigy whose convergence becomes slow after a few initial
iterations.
While Prodigy eventually reaches a similar accuracy to the best methods, it is
much slower at the beginning of the process.
As $p$ increases, our method converges significantly faster than DoG.
We suspect that this improvement arises because our method adapts to the
high-order
smoothness of the function, whereas DoG's convergence rate remains unchanged
and does not take advantage of this property.

In contrast, both DADA and UGM demonstrate stable and consistent performance
across different values of $p$, with DADA performing slightly better than UGM.


==> Preliminaries/discussion_on_c.tex <==
\paragraph{How to choose the constant $c$.}
According to \cref{thm:main-theorem}, our method converges for any
$c > \sqrt{2}$. However, the choice of $c$ can influence the constant factor
in the complexity of DADA. Hence, our goal here is to find the optimal constant
$c$ that minimizes $T_v(\delta)$.
To determine this $c$, let $\bar{r}$ be sufficiently small, so that
\[
  \bar{D}
  \equiv
  \max\Bigl\{ \bar{r}, \frac{2c}{c - \sqrt{2}}D_0 \Bigr\}
  =
  \frac{2c}{c - \sqrt{2}}D_0.
\]
Then, disregarding the logarithmic factors,
due to their minimal impact on the complexity of our method,
we can determine the optimal constant $c$ that minimizes
\begin{align*}
  D
  \equiv
  \sqrt{2} \Bigl( c D_0 + \frac{1}{c} \bar{D} \Bigr)
  =
  \sqrt{2} \Bigl( c + \frac{2}{c - \sqrt{2}} \Bigr) D_0.
\end{align*}
This is the value
\begin{align}\label{eq:optimal-c}
  c = 2\sqrt{2}.
\end{align}
For this optimal choice of $c$, we get $\bar{D} = \max \{\bar{r}, 4 D_0\}$ and
$D = 4 D_0 + \frac{1}{2} \bar{D}$, so the complexity of our method given by
\cref{thm:main-theorem} is
\[
  T_v(\delta) =
  \frac{e^2 (4 D_0 + \frac{1}{2} \bar{D})^2}{\delta^2}
  \log^2 \frac{e \bar{D}}{\Bar{r}}.
\]

